Is Image Memorability Prediction Solved?

This paper deals with the prediction of the memorability of a given image. We start by proposing an algorithm that reaches human-level performance on the LaMem dataset - the only large scale benchmark for memorability prediction. The suggested algorithm is based on three observations we make regarding convolutional neural networks (CNNs) that affect memorability prediction. Having reached human-level performance we were humbled, and asked ourselves whether indeed we have resolved memorability prediction - and answered this question in the negative. We studied a few factors and made some recommendations that should be taken into account when designing the next benchmark.

==> Section5.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% section: Insights on measuring memorability %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{ Insights on measuring memorability}
\label{sec:measures}

Image memorability is commonly measured using an approach that was originally proposed by Isola \etal~\cite{isola2011makes}.
Briefly, the participants are asked to play a ``memory game'' in which images are viewed for a short period  of time and the user is asked to press a button when an image repeats itself.
Memorability is defined as the percentage of correct detections by participants.
%regards as how often the participants tend to correctly detect a repetition of the image. 
%Image memorability can be considered as a population density estimator because it ignores trial-by-trial variability, effectively averaging over a population of participants or experiments \cite{bylinskii2015intrinsic}.
% we assigned a ‘memorability score’ to each target image, as defined in \cite{isola2014makes} as the percentage of correct detections by participants.
By randomizing the sequence each participant sees, the measurements depend only on factors that are intrinsic to the image, independent of extrinsic variables, such as display order, time delay, and local visual context. 
% ince motivation, attention, and participant ability are all known to modulate raw memory performance, memorability is analyzed using rank scores, which should be more stable across changes in user focus and ability.
To evaluate human consistency, Spearman's rank correlation is utilized across different participant groups. 

While in general the game is clever and efficient, we have found three modifications that will make the results even more indicative.
We enumerate them below and elaborate on each of them thereafter.
\begin{enumerate}
\item
Memorability scores for images are meaningful when there are $\geq\!100$ viewers per image, while current datasets use $\approx\!40$.
\item
The order in which the images are displayed to the viewer has a dramatic impact on image memorability.
This should be taken into account when designing an experiment.
%\item
%Some images have a significantly higher variance of memorability scores across people than others. This suggests  that memorability should be represented by both the mean memorability and the variance, whereas currently only the mean is considered.
\item
\shay{
It suffices to maintain only the memorability score.
The variance across observers depends on the memorability score.
Images have a significantly lower variance of memorability scores across people as their average memorability increases. 
%This should be taken into account when designing an experiment.
}
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Number of observers}
\label{subsec:observers}
\ayellet{Lihi, I am not sure i was convinced by the first two paragraphs. what do you think?}
\lihi{I rephrased a bit - I hope I clarified it. There was a bit of confusion in the text.}

% 1. Describe the practice
As image memorability is a subjective attribute, it varies across observers.
Consistency between human observers is important for the memorability scores to be both meaningful and useful for prediction.
Recall that the memory game takes as scores the mean memorability over multiple participants. 
A key question then is how many participants should attend the game for the mean scores to be meaningful?
Isole \etal~\cite{isola2011makes} show that as the number of participants increases, the mean scores become more stable.
To prove stability they show that averaging memorability scores over groups of $40$ participants yields Spearman rank correlation of $\rho=0.75$ between different groups (on the SUN Memorability dataset).
Similarly, Khosla \etal~\cite{khosla2015understanding} measured rank correlation of $\rho=0.68$ on the Lamem dataset, and Bylinskii \etal~\cite{bylinskii2015intrinsic} measured rank correlation of $\rho=0.74$  on the Figrim dataset.

%2. What we did to challenge the above
One problem with these results is that they ignore the standard deviation of the correlation when computed over different splits into groups. 
That is, how stable are the rank correlations between groups?
As it turns out, the variability across splits is quite large, measured at $\sigma=0.2$ on Figrim~\cite{bylinskii2015intrinsic}.
This raises questions regarding the use of memorability scores for prediction, since falling within the variance should be considered as success.
We therefore aim at studying the best group size needed for consistent image memorability scores.

We repeated the same Visual Memorability Game, as described in Section~\ref{subsec:memoryGame}, using target and filler images randomly selected from the Figrim dataset~\cite{bylinskii2015intrinsic}.
In particular, we measured memorability for 45 target images, each scored by 275 participants on average.
We evaluate human consistency across different group sizes as follows.
The participants were split into two equal-size groups and the mean score per image was computed for each group.
We then computed the Spearman’s rank correlation between the scores of the two groups.
This was done for 100 random splits into groups.
We then computed both the mean and the variance of the correlation scores over all splits.

%==================== Technical details====================
%We also measured image variance.
%This human consistency was evaluated for different number of scores per image (10-80). 
%We analyzed the results both by Spearman's rank correlation and by standard deviation measures.
%In order to evaluate memorability variance per image, we randomly selected 100 equal groups of participants, for each memorability score was calculated. Then, average memorability and SD measures were calculated over all groups scores.
%Although raw memory scores were expected to be less stable across observers than rank scores \cite{isola2014makes}, we used it also in order to examine memorability of a single image.
%========================================================

%3. Our experiment results
Figure~\ref{fig:consistency} shows our results. 
For groups of $40$ participants, the consistency is $\rho=0.74$ with standard deviation of $\sigma=0.12$ (compared to $0.74$, $0.2$ respectively in~\cite{bylinskii2015intrinsic}).
%which measured 0.74 (SD:0.2).
For groups of $100$ participants, the consistency significantly increases to $0.86$ ($\sigma=0.07$).
For groups of $135$ participants, the it only slightly increases further to $0.88$ ($\sigma=0.05$).

%4. What we suggest
We conclude that assigning memorability scores should be performed by averaging over at least $100$ participants.
Since collecting memorability measurements for large numbers of participants requires a great deal of work, using $100$ observers seems like a good compromise. 
%We studied the effect the group size on the consistency of the scores.
%Not only have we shown that the consistency increases with the number of observers, but we also recommend to collect measurements from 100 participants, which result in  $\rho=0.86$ (\(SD:0.1\)) correlation.


\begin{figure}[htb]
\centering
%  \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=0.4\textwidth]{correlation_vs_participants02.jpg}
%    \caption{Average memorability variance vs. number of participants}
    %\label{fig:1}
%  \end{subfigure}

%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=\textwidth]{variance_vs_participants02.jpg}
%    \caption{Rank correlation vs. number of participants}
    %\label{fig:2}
%  \end{subfigure}
\caption{{\bf Memorability consistency across groups of participans.} 
Using groups of $100$ participants is a good compromise between the accuracy of human consistency  and the complexity of collecting the data.}
\label{fig:consistency}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Display order}
\label{subsec:order}
%1. Describe the practice
Image memorability is commonly measured across random sequences of images, as described before, in order to isolate extrinsic 
%visual 
effects of image memorability.
Is that the right practice?
Should an image be assigned a single memorability score?
In real life, images are always displayed in some context; for example, when looking at the newspaper, or walking in a museum, the images intentionally appear in a certain order.
In the street, the order of images is not intentional, but it definitely  influences the scenes and objects we will remember or forget.

%2. Challenge #1
We first want to assess the effect of image order on memorability.
We designed a new version of the ``Memory Game'', in which the only difference is that rather than randomly creating image sequences, we used fixed sets of sequences.
For a fixed set of target and filler images (120 altogether), we created 5 orders.
The 120 images were randomly chosen from Figrim.
%  21 target images.

% \ayellet{ All these numbers are very small and contradict the previous subsection.}
This experiment was performed with two ordered sets.
On average, each target image in each sequence, was scored by 55 participants.
We measure consistency between groups of 25 participants.
The correlation between groups when shown sets of different order is low $\rho=0.4$,$\sigma=0.2$, 
while the correlation when shown the same order is high $\rho=0.7$,$\sigma=0.1$.

%3. Our experiment results
To understand why this is the case, see Figure~\ref{fig:displayOrder}, which shows one example, in which the memorability scores within each sequence are consistent ($0.67$ \& $0.58$), but the consistency between these two sequences is very low ($0.1$).
The Figure shows the target images in the order presented to the participants, skipping the fillers.
Take for example, the kitchen scene. 
When presented after different scenes (a), its memorability score is $0.66$, however, when presented after a sequence of bedrooms (b), its memorability score jumped to $0.98$.

We note that in~\cite{bylinskii2015intrinsic} another extrinsic effect was studied---image context, where context is defined as the images the dataset contains.
Our study adds a new facet of context---not only the dataset as a whole, but also the order in which the images are presented, affect memorability and should be considered.

This raises the question of how memorability should be measured.
It may well be the case that the current practice of random orders is the right way to somehow alleviates the influence of this extrinsic effect.
% seq 4- 0.67
% seq 5-0.58
% seq 4-5 - 0.1
\begin{figure*}[!ht]
\centering
  \begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{display_order_seq_4.png}
%    \caption{{\bf Display order 1.}     Images with their memorability scores (Mem) and standard deviation (SD).}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
    \includegraphics[width=\textwidth]{display_order_seq_5.png}
%    \caption{{\bf Display order 2.}     Images with their memorability scores (Mem) and standard deviation (SD).}
  \end{subfigure}
\centering\caption{{\bf Display order affects image memorability.} 
This figure shows the target images from two different orders of the same set of images (target and fillers), along with heir memorability scores (Mem) and the standard deviation (SD).
Depending on the context, the memorability score can dramatically change, e.g. the kitchen.
Conversely, the lighthouse, which is unique in both sequences, get the same memorability score.
}
\label{fig:displayOrder}
\end{figure*}
% \shay{
% In addition, we find high correlation of $0.62$, between a specific order sequence rank scores and those which was measured over all sequences together (similar to the random setting). 
% This observation show that although display order has a big influence on memorability, we don't have to measure memorability for each sequence order separately, but rather measuring it across different order sequences yield similar results. 

% Since measuring memorability for each sequence order separately requires a great deal of work, measuring memorability across different order sequences is a good compromise.
% Future work should try measuring memorability of an image in a specific context more accurately (potentially by $8\%$) by considering the sequence order.
% }

\subsection{Image variance}
\label{subsec:variance}
%
%1. Describe the practice
Previous work assumed that it suffices to characterize an image by a single memorability score, which indicates how often participants correctly detect a repetition of the image.
Is this the right practice? 
How do the memorability scores vary across groups of observers?
In this study we wanted to examine the role of the variance.

%2. What we did to challenge the above
To answer these questions, we measured the variance of the memorability scores given by different groups of people, per image.
The scores were computed by averaging on varying numbers of participants --- from $40$ to $130$.
We measured the variance across groups.
This was done for 45 images.
%, described in Section~\ref{subsec:observers}.

%3. Our experiment results
Figure~\ref{fig:variance} shows our results.
Every point in the graph represents a different image.
A couple conclusions can be drawn from this graph, as follows.
First, the variance depends on the memorability. 
The more memorable an image is, the smaller the variance.
It means that people tend to agree on what makes an image memorable.
Second, the larger the number of participants, the smaller the memorability variance. 
This supports our observation from Section~\ref{subsec:observers}.

%4. What we suggest
While the second observation was expected, the first one was rather surprising.
When we started the study, we believed that the variance will tell us a different story than the memorability score, and both would have to be maintained.
However, Figure~\ref{fig:variance} proves that it suffices to maintain only one number---the memorability score---which is what is the common practice.


\begin{figure}[!ht]
\includegraphics[width=0.4\textwidth]{variane_vs_mean.jpg}
\centering\caption{{\bf Memorability variance depends on memorability score.} Variance decreases as memorability score increases. Variance also decreases for a larger participants group size (K).}
\label{fig:variance}
\end{figure}

